Open-set object detection: towards unified problem formulation and benchmarking

In real-world applications where confidence is key, like autonomous driving, the accurate detection and appropriate handling of classes differing from those used during training are crucial. Despite the proposal of various unknown object detection approaches, we have observed widespread inconsistencies among them regarding the datasets, metrics, and scenarios used, alongside a notable absence of a clear definition for unknown objects, which hampers meaningful evaluation. To counter these issues, we introduce two benchmarks: a unified VOC-COCO evaluation, and the new OpenImagesRoad benchmark which provides clear hierarchical object definition besides new evaluation metrics. Complementing the benchmark, we exploit recent self-supervised Vision Transformers performance, to improve pseudo-labeling-based OpenSet Object Detection (OSOD), through OW-DETR++. State-of-the-art methods are extensively evaluated on the proposed benchmarks. This study provides a clear problem definition, ensures consistent evaluations, and draws new conclusions about effectiveness of OSOD strategies.

==> tables/comparison.tex <==
% \centering
% \caption{Comparison of Methods for Open World Object Detection}
% \label{tab:comparison}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{l|c|c|c|c|c|c}
% \textbf{Method} & \textbf{Pseudo-labeling} & \textbf{Addresses UNKs via} & \textbf{Requires UNK Label} & \textbf{Feature-Based UNKs} & \textbf{Energy/Probability-based} & \textbf{Implementation Notes} \\
% \hline
% OpenDet \cite{OpenDet} & $\times$ & Low-Density Regions & $\times$ & $\times$ & $\checkmark$ & Official Impl. \\
% ORE \cite{OWOD} & $\checkmark$ & Energy Score & $\checkmark$ & $\times$ & $\checkmark$ & Calibrated on Knowns \\
% MAVL \cite{MAVL} & $\checkmark$ & MViT & $\times$ & $\checkmark$ & $\times$ & Pre-trained model \\
% OW-DETR \cite{OW-DETR} & $\checkmark$ & Top Proposals & $\times$ & $\checkmark$ & $\times$ & Partial Impl. \\
% \hline
% Our Method & & & & & & \\
% \end{tabular}
% }

\centering
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\textbf{Method} & \textbf{Detector} & \textbf{Problem Type} & \textbf{External Dataset} & \textbf{R-ULabel} & \textbf{Pre-calibration} & \textbf{SsB} & \textbf{PsL} & \textbf{Probability-based} \\
\hline
VOS \cite{VOS} & Faster-RCNN & OOD & $\times$ & $\times$ & $\checkmark$ & $\times$ & $\times$ & $\checkmark$ \\[2mm]
SIREN \cite{SIREN} & \parbox{2cm}{\centering \baselineskip=10pt Faster-RCNN \\ D-DETR} & OOD & $\checkmark$ & $\times$ & $\checkmark$ & $\checkmark$ & $\times$ & $\checkmark$ \\[2mm]
OpenDet \cite{OpenDet} & \parbox{2cm}{\centering \baselineskip=10pt Faster-RCNN \\ D-DETR} & OSOD & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\checkmark$ \\[2mm]
ORE \cite{OWOD} & Faster-RCNN & OWOD & $\times$ & $\checkmark$ & $\checkmark$ & $\times$ & $\checkmark$ & $\checkmark$ \\
MAVL \cite{MAVL} & MViT & OWOD & \parbox{2cm}{\centering VisualGenome \\ Flickr-30k} & $\times$ & $\times$ & $\times$ & $\checkmark$ & $\times$ \\
OW-DETR \cite{OW-DETR} & D-DETR & OWOD & $\times$ & $\times$ & $\times$ & $\checkmark$ & $\checkmark$ & $\times$ \\
\hline
RobustDet (our) & D-DETR & ROD & $\times$ & $\times$ & $\times$ & $\checkmark$ & $\checkmark$ & $\times$ \\
\end{tabular}
}









